Entity Projection via Machine Translation for Cross-Lingual NER

Although over 100 languages are supported by strong off-the-shelf machine translation systems, only a subset of them possess large annotated corpora for named entity recognition. Motivated by this fact, we leverage machine translation to improve annotation-projection approaches to cross-lingual named entity recognition. We propose a system that improves over prior entity-projection methods by: (a) leveraging machine translation systems twice: first for translating sentences and subsequently for translating entities; (b) matching entities based on orthographic and phonetic similarity; and (c) identifying matches based on distributional statistics derived from the dataset. Our approach improves upon current state-of-the-art methods for cross-lingual named entity recognition on 5 diverse languages by an average of 4.1 points. Further, our method achieves state-of-the-art F_1 scores for Armenian, outperforming even a monolingual model trained on Armenian source data.

==> sections/abstract.tex <==
% Cross-lingual approaches for natural language processing 
% leverage data from annotation-rich languages like English 
% to solve downstream tasks in under-resourced languages. 
% This paper focuses on cross-lingual \emph{named entity recognition} 
% % building upon previous annotation projection techniques.
% for medium-resource languages that have off-the-shelf MT systems.
% % that combine machin  e translation and entity projection 
% % Z: Perhaps too granular for the abstract?
% % (entity alignment and tag projection), 
% % with promising results. 
% We propose the Translate-Match-Project method (TMP) that:
Cross-lingual approaches for natural language
processing leverage data from annotation-rich
languages like English to solve downstream
tasks in under-resourced languages. 
This paper focuses on cross-lingual \emph{named entity
recognition}, building upon previous annotation projection techniques. 
We propose a system that improves over prior entity-projection methods by:
(a) leveraging machine translation systems twice: 
first for translating sentences and subsequently for translating entities;
(b) matching entities based on orthographic and phonetic similarity; 
and (c) identifying matches based on distributional statistics derived from the dataset. 
The proposed approach improves state-of-the-art 
for cross-lingual named entity recognition on 
$5$ diverse languages by an average of $4.1$ points. 
Further, our method achieves state-of-the-art $F_1$ scores for Armenian, outperforming even a monolingual model trained on Armenian source data.
    
% and (c) identifying matches based on distributional statistics 
% derived from the dataset. 


% Cross-lingual approaches for Natural Language Processing (NLP) utilize data in annotation-rich languages like English to solve NLP tasks in other languages. In this paper, we focus on cross-lingual Named Entity Recognition (NER). For this task, projection-based techniques that use Machine Translation (MT) followed by entity projection (entity alignment and tag projection) have shown the most promising results. However, these methods suffer from noise in the entity projection step. In this work, we demonstrate that projection can be performed more effectively by (a) leveraging state-of-the-art MT systems twice: first for translating sentences and then for translating entities and (b) matching entities based on orthographic and phonetic similarity and distributional statistics derived from the dataset. The proposed approach achieves state-of-the-art results for cross-lingual NER on a diverse set of annotation-poor languages.
    
    
 % Cross-lingual approaches for Natural Language Processing (NLP) utilize data in annotation-rich languages like English to solve NLP tasks in other languages. In this paper, we focus on cross-lingual Named Entity Recognition (NER). For this task, projection-based techniques that use Machine Translation (MT) followed by entity projection (entity alignment and tag projection) have shown the most promising results. However, these methods suffer from noise in the entity projection step. In this work, we demonstrate that projection can be performed more effectively by (a) leveraging state-of-the-art MT systems twice: first for translating sentences and then for translating entities and (b) matching entities based on orthographic and phonetic similarity and distributional statistics derived from the dataset. The proposed approach achieves state-of-the-art results for cross-lingual NER on a diverse set of annotation-poor languages.
    
    
    %We demonstrate that this approach helps achieve state-of-the-art results for cross-lingual NER on several medium-to-low resource languages by matching affixes based on 
    
    % 1) There are very few languages for which annotated data is available for NER.
    % 2) Past approaches consist of direct transfer or projection-based approaches
    % 3) Projection-based approaches rely on either word-level translation or sentence-level translation using an existing Machine Translation (MT) systems, followed by heuristic alignment methods.
    % 4) These heuristic alignment methods are very noisy.
    % 5) We demonstrate that alignment can be achieved more effectively by (a) leveraging MT twice: first for obtaining sentence translations and then for obtaining translations for entities and then (b) by matching source entities to their translations in the target language. We demonstrate that this approach helps achieve state-of-the-art results for cross-lingual NER on several medium-to-low resource languages.
    
% Despite the progress in cross-lingual approaches to \emph{named entity recognition}, there still exist ov

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

Despite rapid advances in statistical tools 
for various NFinally, although our method beats state-of-the-art baselines, it lags behind the NER model trained on large monolingual corpora. This could possibly be due to domain shift (as evidenced by improvement in Hindi $F_1$ in Parallel regime), handling which, could be a promising future direction. Natural Language Processing (NLP) tasks,
the benefits of this technology accrue disproportionately 
to those working with languages, like English,
for which large annotated corpora exist.
For any given task, e.g. Named Entity Recognition (NER) or Semantic Role Labeling (SRL), 
owing to the dependence of state-of-the-art deep learning approaches 
on large numbers of training examples,
creating suitable datasets can be prohibitively expensive.
This asymmetry between high- and low-resource languages
has inspired work on cross-lingual approaches,
utilizing annotated data from resource-rich languages 
to build strong models for (comparatively) low-resource languages. 


We focus on cross-lingual approaches to NER
owing to the importance of NER models as core components 
in \emph{information retrieval} and \emph{question answering} sytems.
NER consists of identifying named entities in a sentence 
such as PERSON (e.g., Barack Obama), LOCATION (e.g., Africa), 
ORGANIZATION (e.g., United Nations), etc.
Recently, a number of papers have made progress on cross-lingual NER,
proposing a variety of mechanisms to facilitate the transfer.
Some approaches directly apply the models trained on English, 
using language-agnostic features,
while projection-based approaches \citep{mayhew2017cheap, xie2018neural, zhang2016bitext, kim2010cross} first
create training sets in the target language,
often through word-by-word translation via dictionaries or aligned word vectors
and then train an NER model in the target language.

% When bitext is available, trained models are used to generate noisy source tags that are then projected
% \citep{mayhew2017cheap, xie2018neural, zhang2016bitext, kim2010cross, pado2009cross}. All these methods are prone to one or more of the following sources of errors: source side annotation noise, translation noise or entity projection noise.



% We are motivated by the need to bridge this asymmetry by leveraging high quality MT.
% However, high-quality MT systems such as Google Translate
% are now available for over 100 languages.

% there is a dearth of performant systems in non-English languages, 
% for say, NER, which is a cornerstone of important applications 
% such as Information Retrieval and Question Answering. 
% While there exist high quality MT systems such as Google Translate for over 100 languages, there is a dearth of performant systems in non-English languages, for say, NER, which is a cornerstone of important applications such as Information Retrieval and Question Answering. 

% This asymmetry, across languages, in access to datasets for training
% has led some researchers to investigate cross-lingual approaches,
% utilizing annotated data from resource-rich languages 
% to solve these tasks in languages that have fewer annotated resources. 
% We are motivated by the need to bridge this asymmetry by leveraging high quality MT.


% There is a greater impetus in advancing MT and there exist high quality MT systems such as Google Translate for over 100+ languages. On the other hand, for tasks like NER, there is a significant gap in performance between English and even medium sourced langauges like Spanish, German. However, NER is important in downstream applications like IR and QA, and therefore its essential to drive progress in tasks like NER even for medium resourced languages. It is a cornerstone of important downstream tasks such as Information Retrieval and QA.
% It is a cornerstone of important downstream tasks such as Information Retrieval and QA. 



% For the translation step, past works have used both word-to-word translations using bilingual lexicons \cite{mayhew2017cheap, xie2018neural} and state-of-the-art MT systems \cite{ni2017weakly}. For the entity projection step, past works have either used alignment methods from statistical MT literature.

% Approaches to cross-lingual NER can be broadly divided into two categories: direct transfer, in which a model trained on the source language is directly applied to the target language and projection-based approaches, in which first data and labels are first transferred from source to target languages and then a model is trained in the target language. Past works have shown that projection-based methods are more effective for cross-lingual NER.

% Projection-based approaches are comprised of two steps: (a) translation of sentences followed by (b) entity projection, i.e., alignment of entities followed by projection of their tags. 



% describing past work not putting in context
% Thus, noise gets added along both these steps.

In this paper, we are motivated by the observation 
that even for languages lacking NER corpora,
high-quality language machine translation (MT) are often available. 
Google Translate, for example, is now available in over $100$ languages.
Our proposed method combines off-the-shelf translation
with a more sophisticated entity projection procedure
to achieve state-of-the art performance for a variety of language pairs. 
Many prior papers on cross-lingual NER
have focused on quick-and-dirty approaches to MT, 
perhaps because the low-resource assumption might appear to preclude available MT systems.
These authors resort to noisy translation 
through word-level or phrase-level lexicons. 
In these works, the entity projection step is easily accomplished,
because the tags can be directly copied.
However, we note that high-quality machine translation is more widely available
than other corpora.
For example, Google Translate provides quality translations from English to Hindi
but no public resources for NER exist in Hindi 
comparable to the CoNLL or OntoNotes datasets. 


One consequence of relying on powerful MT
is that corresponding translated sentences 
may not be aligned word-for-word with the originals.
From English to French, ``My feet hurt'' becomes ``J'ai mal au pied'' 
(something more like ``I have pain at the foot''). 
Thus, with powerful MT, entity projection requires aligning words.
% between an original example and its translation,     
has been studied in the context of statistical MT \cite{koehn2003statistical}, 
but has received less attention in the context of cross-lingual entity projection.
% that require a selective projection of entities across sentences. 

% We attempt to fill this research gap.
% uts solving something harder, less frewuent entities are harder to align its supervised 

% MT based alignment methods have been adopted to selectively project named entities \cite{mayhew2017cheap}, but are noisy. 
% which are already available for several annotation-poor languages, 
% because we hypothesize that word order differences are crucial for cross-lingual NER, especially for languages distant from English. 



Hypothesizing that the poor quality of word-for-word translations 
hinders previous cross-lingual NER systems,
Our methods leverage production-level MT systems 
by (a) leveraging MT systems twice: 
first for translating sentences and then for translating entities;
(b) matching entities based on orthographic and phonetic similarity;
and (c) identifying matches based on distributional statistics 
derived from the dataset. 
Our proposed method achieves state-of-the-art results 
for cross-lingual NER on $4$ different annotation-poor languages. Averaged across languages, our model achieves a $3.87$ gain in F1 over the previous state-of-the-art.

% pass the entities as individual phrases to be translated. We then solve the task of "locating" these translated entities in the translated sentence in the following manner: a) phonetic and orthographic affix matching b) word-edit distance based maximal sub sequence based entity matching and c) distributional statistics based entity matching. We show that this technique is better than the alignment techniques used for MT and as a result we are able to get state-of-the-art on 5 different languages. 
% We comapre against really strong baselines
% We ablate to uncover the gains of each of our additions to the technique

% \textbf{Contributions:} In our paper, we focus on languages for which translation systems exist currently and we minimize noise in the translation process by utilizing state-of-the-art translation systems. We propose an entity projection method, that improves and we achieve sota performance on 5 languages: Spanish, Dutch, German, Hindi and Tamil.
% Our contributions are :
% \begin{itemize}
%     \item We leverage state of the art MT along with our novel technique to selectively align and project source entities to the translated target sentence to push performance on NER for 5 languages beyond the current state-of-the-art.
% \end{itemize}

% Progress in statistical approaches to Natural Language Processing in the last several years has been concentrat

% Over the last many years, neural approaches have achieved state-of-the-art results for several Natural Language Processing (NLP) tasks such as Named Entity Recognition \cite{lample2016neural}, Natural Language Inference, Question Answering \cite{devlin2018bert}, etc. However, their adoption in non-English languages has been slow due to their heavy dependence on a significant amount of annotated resources, which are difficult to obtain due to the prohibitive cost (time, money and expertise) of annotation.

% 1) Over the last several years, statistical approaches have emerged as the paradigm of choice for NLP. / They have achieved state-of-the-art results for several NLP tasks.
% 2) However, since these approaches require a lot of data and collecting data is expensive, in terms of time, money and expertise, these gains have been largely restricted to English.




% which is currently unavailable for non-English languages due to the prohibitive cost of annotation. 

% tasks such as Named Entity Recognition (NER)

% (1) Introduce cross-lingual NLP
% (2) Focus on cross-lingual NER
% (3) Explain various methods, justify why we choose projection-based methods
% (4) Explain the problem of projection-based methods
% (5) Explain how we solve it
% (6) Give a glimpse of the results

% All of this needs to fit within the first page.
